Minimizing Age-of-Information with Throughput Requirements in Multi-Path Network Communication

We consider the scenario where a sender periodically sends a batch of data to a receiver over a multi-hop network, possibly using multiple paths. Our objective is to minimize peak/average Age-of-Information (AoI) subject to throughput requirements. The consideration of batch generation and multi-path communication differentiates our AoI study from existing ones. We first show that our AoI minimization problems are NP-hard, but only in the weak sense, as we develop an optimal algorithm with a pseudo-polynomial time complexity. We then prove that minimizing AoI and minimizing maximum delay are "roughly" equivalent, in the sense that any optimal solution of the latter is an approximate solution of the former with bounded optimality loss. We leverage this understanding to design a general approximation framework for our problems. It can build upon any $\alpha$-approximation algorithm of the maximum delay minimization problem, to construct an $(\alpha+c)$-approximate solution for minimizing AoI. Here $c$ is a constant depending on the throughput requirements. Simulations over various network topologies validate the effectiveness of our approach.

==> challenge.tex <==
\section{Our Problems are Challenging} \label{sec:challenge}
As discussed in Sec.~\ref{sec:introduction}, in the literature there are two multi-path routing problems that are highly relevant to \textsf{MPA} and \textsf{MAA}, and thus to \textsf{MPA-T} and \textsf{MAA-T}. They are the quickest flow problem and the maximum latency problem, and are special cases of \textsf{MMD} (thus of \textsf{MPA} and \textsf{MAA}, too, according to Lem.~\ref{lem:age-delay}). In this section, we show that conceivable extensions of them output suboptimal solutions to \textsf{MPA} and \textsf{MAA}, where the optimality gap can be unacceptable for time-sensitive applications. Thus developing efficient algorithms for our \textsf{AoI} minimization problems are uniquely challenging.
\subsection{The Quickest Flow Problem}
The quickest flow problem~\cite{lin2015quickest} is a special case of \textsf{MMD} when $T=+\infty$. If we directly use its optimal solution as the solution to \textsf{MPA} and \textsf{MAA}, the achieved \textsf{AoI} can be suboptimal, because that the quickest flow problem does not consider that the transmission of data from different tasks with distinct starting times may share the link at certain time. Specifically, we have the following Thm.~\ref{thm:DF-MPA}   
\begin{figure}[]
	\centering
	\includegraphics[width=0.45\columnwidth]{fig/TwoLinks.pdf}
	\caption{A simple network with two nodes and two parallel links. We assume the delay of $e_1$ (resp. $e_2$) is 1 (resp. 3). We assume unit bandwidths for both links. We assume $R=2$.}
	\label{fig:two-links}
\end{figure}

\begin{theorem}\label{thm:DF-MPA}
Given an arbitrary instance of \textsf{MPA}, i.e., given a network $G(V,E)$, a sender $s\in V$, a receiver $r\in V\backslash\{s\}$, a task period $T\in\mathbb{Z}^+$, and a throughput requirement $R>0$, suppose this \textsf{MPA} instance is theoretically feasible. Then it holds that the corresponding quickest flow problem instance, which is defined by the same $G$, $s$, $r$, and $R$, must be theoretically feasible. Moreover, suppose $f_q$ is the optimal solution to this quickest flow problem, then it holds that (i) either $f_q$ is infeasible to this \textsf{MPA}, or (ii) $f_q$ is optimal to this \textsf{MPA}.
\end{theorem}
\begin{proof}
	The existence of $f_q$ comes from that any feasible solution to the \textsf{MPA} is a feasible solution to the corresponding quickest flow problem. The existence of instances where $f_q$ is infeasible to \textsf{MPA} can be proved by the representative example of Fig.~\ref{fig:two-links}. The optimality of $f_q$ when it is feasible to \textsf{MPA} can be proved straightforwardly by contradiction.  Details are referred to Appendix~\ref{subsec:DF-MPA}.
\end{proof}

Thm.~\ref{thm:DF-MPA} suggests that the optimal solution to the quickest flow problem is either (i) infeasible to \textsf{MPA} (\textsf{MAA}), and thus leading to an unbounded peak (average) \textsf{AoI}, or (ii) optimal to \textsf{MPA} (\textsf{MAA}). Due to the unbounded \textsf{AoI} performance, the direct extension of the quickest flow problem outputs unacceptable \textsf{AoI}s for certain instances of our \textsf{AoI} minimization problems. 

\subsection{The Maximum Latency Problem}
The maximum latency problem~\cite{misra2009polynomial} is a special case of our \textsf{MMD} when $T=1$. Let us denote the optimal solution to the maximum latency problem with a throughput $R$ as $\textsf{MLP}(R)$. In the following we show that one conceivable extension of the maximum latency problem can obtain suboptimal solutions to \textsf{MPA} and \textsf{MAA}.
\begin{figure}[]
	\centering
	\includegraphics[width=0.45\columnwidth]{fig/OneLink.pdf}
	\caption{A simple network with two nodes and one link. We assume $d_e=1$ and $b_e=R=10$.}
	\label{fig:one-links}
\end{figure}

Recall that in our scenario, there is $R$ amount of data arriving at $s$ at each time $t=kT,\forall k\in\mathbb{Z}$, waiting for transmission. A relevant scenario in the maximum latency problem is that there is $R/T$ amount of data arriving at $s$ at each time $t,\forall t\in\mathbb{Z}$. Different from Thm.~\ref{thm:DF-MPA} which proves that the optimal solution to the quickest flow problem can be infeasible to \textsf{MPA}, here it is straightforward that the solution of $\textsf{MLP}(R/T)$, i.e., the optimal solution to the maximum latency problem with throughput $R/T$, must be a feasible solution to \textsf{MPA}, but this solution requires to hold certain amount of data at $s$ at each time from the perspective of \textsf{MPA}. We remark that the \textsf{AoI} performance of $\textsf{MLP}(R/T)$ can be suboptimal (see the following Thm~\ref{thm:MLP-AOI}) for \textsf{MPA} (thus for \textsf{MAA}), because that this solution always streams $R/T$ amount of data to the network at each time, and it ignores that we can stream various amount of data to the network at different time offsets in our \textsf{AoI} minimization scenario.

In order to prove Thm~\ref{thm:MLP-AOI}, we first give a lemma bellow.

\begin{lemma}\label{lem:MLP}
	Given an arbitrary instance of \textsf{MPA}, i.e., given a network $G(V,E)$, a sender $s\in V$, a receiver $r\in V\backslash\{s\}$, a task period $T\in\mathbb{Z}^+$, and a throughput requirement $R>0$, suppose this \textsf{MPA} instance is feasible. Then it holds that the corresponding maximum latency problem instance, which is defined by the same $G$, $s$, $r$, but with a throughput requirement of $R/T$, must be feasible. Moreover, suppose $f_p$ (resp. $f_m$) is the optimal solution to the \textsf{MPA} instance (resp. to the maximum latency problem instance), we have that $f_m$ must be feasible to \textsf{MPA}, and the following holds in the view of \textsf{MPA}
	\be
	\mathcal{M}(f_p)~\ge~ \mathcal{M}(f_m)-T+1.\nnb
	\ee
\end{lemma}
\begin{proof}
	The lemma holds because for any feasible periodically repeated solution to \textsf{MPA} with throughput $R$, we can construct a feasible solution to the corresponding maximum latency problem with throughput $R/T$. Details are referred to Appendix~\ref{subsec:MLP}. 
\end{proof}

Now with Lem.~\ref{lem:MLP}, we have the following Thm.~\ref{thm:MLP-AOI}.

\begin{theorem}\label{thm:MLP-AOI}
	Given an arbitrary instance of \textsf{MPA} (\textsf{MAA} equivalently) with a throughput requirement $R>0$ and a task period $T\in\mathbb{Z}^+$, suppose $f_p$ (resp. $f_a$) is the optimal solution to this \textsf{MPA} (resp. \textsf{MAA}). Then it holds that the optimal solution $f_m$ to the corresponding maximum latency problem instance with a throughput requirement $R/T$ must exist, and it must be a feasible solution to the \textsf{MPA} and \textsf{MAA}, with the following bounded \textsf{AoI} gaps guaranteed
	\bee
	&& \Lambda_p(f_m)/\Lambda_p(f_p)~\le~2,\label{eqn:2-gap}\\
	&& \Lambda_a(f_m)/\Lambda_a(f_a)~\le~3.\label{eqn:3-gap}
	\eee
	Moreover, both gaps are tight, in the sense that there exist instances where $\Lambda_p(f_m)/\Lambda_p(f_p)$ is arbitrarily close to $2$ and $\Lambda_a(f_m)/\Lambda_a(f_a)$ is arbitrarily close to $3$. 
\end{theorem}
\begin{proof}
	The correctness of this theorem can be proved based on Lem.~\ref{lem:MLP}, and the tightness can be proved using the instance of Fig.~\ref{fig:one-links}. Details are referred to Appendix~\ref{subsec:MLP-AOI}.
\end{proof}

Thm.~\ref{thm:MLP-AOI} suggests that the conceivable extension of the maximum latency problem, i.e., $\textsf{MLP}(R/T)$, provides a $2$-approximation algorithm for solving \textsf{MPA} and a $3$-approximation algorithm for solving \textsf{MAA}. Moreover, there exist instances where the achieved optimality gaps are arbitrarily close to the approximation ratios. Considering that the approximation ratio $2$ on the peak \textsf{AoI} and $3$ on the average \textsf{AoI} are too large to be acceptable especially for time-sensitive applications, this conceivable extension is not a desired approach for our \textsf{AoI} minimization problems.

\begin{comment}
Another method of using \textsf{ALGO} to solve \textsf{MPA} is to round and scale the input network $G$. Considering that $T=1$ in the maximum latency problem, for \textsf{MPA} with an arbitrary period $T\ge 1$, we can round the period $T$ as a unit of time $T/T=1$. With this scaling and rounding technique where one time slot after rounding is equivalent to $T$ time slots before rounding, it is clear that for each link $e\in E$, we shall further round the link delay to $\hat{d}_e=\lceil d_e/T\rceil$ and round the link bandwidth to $\hat{b}_e=b_e\cdot T$. Thus we can obtain a rounded network $\hat{G}$ that has the same topology as $G$ but has different link delays and link bandwidths. And we can use the solution of $\textsf{ALGO}(\hat{G},R)$ as a solution to \textsf{MPA}. However, we remark that $\textsf{ALGO}(\hat{G},R)$ outputs suboptimal solutions to \textsf{MPA}, mainly due to the following two reasons. (1) The link delay changes and thus is not the exact input delay during the rounding of $\hat{d}_e=\lceil d_e/T\rceil$. (2) Since the exact bandwidth of $e=(v,w)$ in $G$ is $b_e$, a delay that varies from $1$ to $T-1$ is incurred in $G$ to hold data at the link source node $v$, when we try to send an amount of data that is greater than $b_e$ to the link $e$. Now in $\hat{G}$, by setting $\hat{b}_e=b_e\cdot T$, we allow $b_e\cdot T$ amount of data to be sent to the link $e$ at each time. But the rounding of $\hat{d}_e=\lceil d_e/T\rceil$ in $\hat{G}$ does not consider those varying data-holding delays that should be incurred in the exact input network $G$.
\begin{figure}[]
	\centering
	\includegraphics[width=0.45\columnwidth]{fig/TwoLinks.pdf}
	\caption{A network with two nodes and two parallel links. We assume a $1$ delay for both links. We assume the bandwidth of $e_1$ (resp. $e_2$) is $1$ (resp. $T$). We assume $R=T$.}
	\label{fig:two-links-latency}
\end{figure}

Let us look at the network in Fig.~\ref{fig:two-links-latency} with an arbitrary large $T$. It is easy to verify that in $\hat{G}$, the rounded delay is $1$ for both links, and the rounded bandwidth is $T$ (resp. $T^2$) for $e_1$ (resp. $e_2$). Thus, one optimal solution of $\textsf{ALGO}(\hat{G},R)$ is to stream all the $R=T$ data to $e_1$. This solution has a peak \textsf{AoI} of $(2T-1)$ and an average \textsf{AoI} of $(3T-1)/2$, but in our problem the optimal peak \textsf{AoI} is $T$ and the optimal average \textsf{AoI} is $(T+1)/2$, by streaming the full data $R=T$ to the link $e_2$ at offset $0$. Thus the peak \textsf{AoI} optimality gap is close to $2$, and the average \textsf{AoI} optimality gap is close to $3$, when $T$ is very large.
\end{comment} 

Overall, we observe that our \textsf{AoI} minimization problems \textsf{MPA}, \textsf{MAA}, \textsf{MPA-T}, and \textsf{MAA-T} are uniquely challenging, because (i) they are all NP-hard, since as a special case of \textsf{MMD}\footnote{Note that \textsf{MMD} is equivalent to \textsf{MPA} and \textsf{MAA} according to Lem.~\ref{lem:age-delay}, and is a special case of \textsf{MPA-T} and \textsf{MAA-T}.}, the maximum latency problem is known to be NP-hard~\cite{misra2009polynomial}. (ii) Moreover, as discussed in this section, conceivable extensions of existing solutions are suboptimal for our problems, where the optimality gap comparing the achieved \textsf{AoI} to the optimal \textsf{AoI} is unacceptable especially for time-sensitive applications.
